Determining vaccine responders in the presence of baseline immunity using single-cell assays and paired control samples

A key objective in vaccine studies is to evaluate vaccine-induced immunogenicity and determine whether participants have mounted a response to the vaccine. Cellular immune responses are essential for assessing vaccine-induced immunogenicity, and single-cell assays, such as intracellular cytokine staining (ICS) are commonly employed to profile individual immune cell phenotypes and the cytokines they produce after stimulation. In this article, we introduce a novel statistical framework for identifying vaccine responders using ICS data collected before and after vaccination. This framework incorporates paired control data to account for potential unintended variations between assay runs, such as batch effects, that could lead to misclassification of participants as vaccine responders. To formally integrate paired control data for accounting for assay variation across different time points (i.e., before and after vaccination), our proposed framework calculates and reports two p-values, both adjusting for paired control data but in distinct ways: (i) the maximally adjusted p-value, which applies the most conservative adjustment to the unadjusted p-value, ensuring validity over all plausible batch effects consistent with the paired control samples' data, and (ii) the minimally adjusted p-value, which imposes only the minimal adjustment to the unadjusted p-value, such that the adjusted p-value cannot be falsified by the paired control samples' data. We apply this framework to analyze ICS data collected at baseline and 4 weeks post-vaccination from the COVID-19 Prevention Network (CoVPN) 3008 study. Our analysis helps address two clinical questions: 1) which participants exhibited evidence of an incident Omicron infection, and 2) which participants showed vaccine-induced T cell responses against the Omicron BA.4/5 Spike protein.

==> old_stuff.tex <==

\subsection{Incorporating the Negative Control into Outcome Testing (Scenario 1)}
 \textcolor{purple}{BZ: We suppose that the assay was run separately for baseline and post-vaccination, and hence different false positive/false negative rates.} \textcolor{purple}{BZ: We are mostly concerned about falsely designating a participant as responding to the vaccine, so the primary focus will be to guard against the bias induced by the batch effect, i.e., the assay run at the post-vaccination timepoint has a higher false positive rate or the assay run at baseline has a higher false negative rate.} Our strategy consists of two steps:
\begin{itemize}

    \item Step 1: Using the negative control to construct a valid $100(1-\alpha_{1})\%$ level confidence region $A_{1-\alpha_{1}}$ for the misclassification rates $(p_{B, 0|1}, p_{B, 1|0}, p_{V, 0|1}, p_{V, 1|0})\in [0,1]^{4}$. Specifically, we let $p^{N}_{B, 1}$ (or $p^{N}_{B, 0}$) denote the true rate of positive (or negative) outcome among the baseline samples from the negative control, and $p^{N}_{V, 1}$ (or $p^{N}_{V, 0}$) the true rate of positive (or negative) outcome among the post-vaccination samples from the negative control. Parallelly, we let $p^{N, *}_{B, 1}$ (or $p^{N, *}_{B, 0}$) denote the expected rate of observing a positive (or negative) outcome among the baseline samples from the negative control, and $p^{N, *}_{V, 1}$ (or $p^{N, *}_{V, 0}$) the expected rate of observing a positive (or negative) outcome among the post-vaccination samples from the negative control. Then we have 
    \begin{equation*}
        p^{N, *}_{B, 1}=p^{N}_{B, 1}\times (1-p_{B, 0|1})+p^{N}_{B, 0}\times p_{B, 1|0}=p^{N}_{B, 1}\times (1-p_{B, 0|1})+(1-p^{N}_{B, 1})\times p_{B, 1|0},
    \end{equation*}
    which implies that 
    \begin{equation*}
        p^{N}_{B, 1}=\frac{p^{N, *}_{B, 1}-p_{B, 1|0}}{1-p_{B, 0|1}-p_{B, 1|0}}.
    \end{equation*}
    Similarly, we have 
     \begin{equation*}
        p^{N}_{V, 1}=\frac{p^{N, *}_{V, 1}-p_{V, 1|0}}{1-p_{V, 0|1}-p_{V, 1|0}}.
    \end{equation*}
  Under fixed $(p_{B, 0|1}, p_{B, 1|0}, p_{V, 0|1}, p_{V, 1|0})$, consider the test statistic 
  \begin{equation*}
      T^{N}=\widehat{p}^{N}_{V, 1}-\widehat{p}^{N}_{B, 1}=\frac{\widehat{p}^{N, *}_{V, 1}-p_{V, 1|0}}{1-p_{V, 0|1}-p_{V, 1|0}}-\frac{\widehat{p}^{N, *}_{B, 1}-p_{B, 1|0}}{1-p_{B, 0|1}-p_{B, 1|0}},
  \end{equation*}
  where $\widehat{p}^{N, *}_{B, 1}$ (or $\widehat{p}^{N, *}_{V, 1}$) denote the sample proportion of positive outcomes among the baseline (or post-vaccination) samples from the negative control. 
  \begin{assumption}\label{assump: independence of negative control}
      The samples from the negative control are independent, either from the baseline or post-vaccination group (i.e., both within-group independence and across-group independence hold). 
  \end{assumption}
  \begin{assumption}[Negative Control]\label{assump: negative control}
      We have $p^{N}_{V, 1}=p^{N}_{B, 1}$, and the negative control samples and study samples from participants share the same values of the four misclassification rates $(p_{B, 0|1}, p_{B, 1|0}, p_{V, 0|1}, p_{V, 1|0})$. 
  \end{assumption}
We have the following theorem:
\begin{theorem}\label{thm: negative control}
    Under Assumptions~\ref{assump: independence of negative control} and \ref{assump: negative control}, as well as the true values of $(p_{B, 0|1}, p_{B, 1|0}, p_{V, 0|1}, p_{V, 1|0})$, we have 
    \begin{equation*}
      \overline{T}^{N}=  \frac{T^N }{\sqrt{\widehat{p}^{N}_{1}(1-\widehat{p}^{N}_{1}) \Big(\frac{1}{N_{1}^{\prime}}+\frac{1}{N_{0}^{\prime}}\Big) } }\xrightarrow{d} N(0,1),
    \end{equation*}
    where 
    \begin{equation*}
        \widehat{p}^{N}_{1}=\frac{N_{1}^{\prime}}{N_{0}^{\prime}+N_{1}^{\prime}}\times \frac{\widehat{p}^{N, *}_{V, 1}-p_{V, 1|0}}{1-p_{V, 0|1}-p_{V, 1|0}}+\frac{N_{0}^{\prime}}{N_{0}^{\prime}+N_{1}^{\prime}}\times \frac{\widehat{p}^{N, *}_{B, 1}-p_{B, 1|0}}{1-p_{B, 0|1}-p_{B, 1|0}}.
    \end{equation*}
\end{theorem}
Therefore, an $100(1-\alpha_{1})\%$ confidence set for $(p_{B, 0|1}, p_{B, 1|0}, p_{V, 0|1}, p_{V, 1|0})$ is 
\begin{equation*}
    A_{1-\alpha_{1}}=\{(p_{B, 0|1}, p_{B, 1|0}, p_{V, 0|1}, p_{V, 1|0})\in [0,1]^{4}: \overline{T}^{N}\in [-z_{1-\alpha_{1}/2}, z_{1-\alpha_{1}/2}] \}.
\end{equation*}

\textcolor{red}{Siyu: If we have additional information or constraints on $(p_{B, 0|1}, p_{B, 1|0}, p_{V, 0|1}, p_{V, 1|0})$, we can add them, or if we have additional information on $p^{N}_{V, 1}$ or $p^{N}_{B, 1}$.}
    

    \item Step 2: We let $p^{(i)}_{B, 1}$ (or $p^{(i)}_{B, 0}$) denote the true rate of positive (or negative) outcome among the baseline samples from the study participant $i$, and $p^{(i)}_{V, 1}$ (or $p^{(i)}_{V, 0}$) the true rate of positive (or negative) outcome among the post-vaccination samples from the study participant $i$. Parallelly, we let $p^{(i), *}_{B, 1}$ (or $p^{(i), *}_{B, 0}$) denote the expected rate of observing a positive (or negative) outcome among the baseline samples from the study participant $i$, and $p^{(i), *}_{V, 1}$ (or $p^{(i), *}_{V, 0}$) the expected rate of observing a positive (or negative) outcome among the post-vaccination samples from the study participant $i$. Then we have 
    \begin{equation*}
        p^{(i), *}_{B, 1}=p^{(i)}_{B, 1}\times (1-p_{B, 0|1})+p^{(i)}_{B, 0}\times p_{B, 1|0}=p^{(i)}_{B, 1}\times (1-p_{B, 0|1})+(1-p^{(i)}_{B, 1})\times p_{B, 1|0},
    \end{equation*}
    which implies that 
    \begin{equation*}
        p^{(i)}_{B, 1}=\frac{p^{(i), *}_{B, 1}-p_{B, 1|0}}{1-p_{B, 0|1}-p_{B, 1|0}}.
    \end{equation*}
    Similarly, we have 
     \begin{equation*}
        p^{(i)}_{V, 1}=\frac{p^{(i), *}_{V, 1}-p_{V, 1|0}}{1-p_{V, 0|1}-p_{V, 1|0}}.
    \end{equation*}
    Under fixed $(p_{B, 0|1}, p_{B, 1|0}, p_{V, 0|1}, p_{V, 1|0})$, consider the test statistic $T^{(i)}$ for testing $H_{0}^{(i)}: p^{(i)}_{V, 1}= p^{(i)}_{B, 1}$, in which
  \begin{equation*}
      T^{(i)}=\widehat{p}^{(i)}_{V, 1}-\widehat{p}^{(i)}_{B, 1}=\frac{\widehat{p}^{(i), *}_{V, 1}-p_{V, 1|0}}{1-p_{V, 0|1}-p_{V, 1|0}}-\frac{\widehat{p}^{(i), *}_{B, 1}-p_{B, 1|0}}{1-p_{B, 0|1}-p_{B, 1|0}},
  \end{equation*}
  where $\widehat{p}^{(i), *}_{B, 1}$ (or $\widehat{p}^{(i), *}_{V, 1}$) denote the sample proportion of positive outcomes among the baseline (or post-vaccination) samples from the participant $i$. 
  \begin{assumption}\label{assump: independence of study samples}
      The samples from the study participant $i$ are independent, either from the baseline or post-vaccination group (i.e., both within-group independence and across-group independence hold). 
  \end{assumption}

  \begin{theorem}\label{thm: study sample}
    Under Assumptions~\ref{assump: independence of study samples} and $H_{0}^{(i)}$, as well as the true values of $(p_{B, 0|1}, p_{B, 1|0}, p_{V, 0|1}, p_{V, 1|0})$, we have 
    \begin{equation*}
      \overline{T}^{(i)}=  \frac{T^{(i)} }{\sqrt{\widehat{p}^{(i)}_{1}(1-\widehat{p}^{(i)}_{1}) \Big(\frac{1}{N_{1}}+\frac{1}{N_{0}}\Big) } }\xrightarrow{d} N(0,1),
    \end{equation*}
    where 
    \begin{equation*}
        \widehat{p}^{(i)}_{1}=\frac{N_{1}}{N_{0}+N_{1}}\times \frac{\widehat{p}^{(i), *}_{V, 1}-p_{V, 1|0}}{1-p_{V, 0|1}-p_{V, 1|0}}+\frac{N_{0}}{N_{0}+N_{1}}\times \frac{\widehat{p}^{(i), *}_{B, 1}-p_{B, 1|0}}{1-p_{B, 0|1}-p_{B, 1|0}}.
    \end{equation*}
\end{theorem}
Therefore, a one-sided $p$-value for testing $H_{0}^{i}$ under true values of $(p_{B, 0|1}, p_{B, 1|0}, p_{V, 0|1}, p_{V, 1|0})$ is $1-\Phi(\overline{T}^{(i)})$.
 
\textcolor{red}{Siyu: How to combine Steps 1 and 2? For example, do we want to minimize $1-\Phi(\overline{T}^{(i)})$ subject to $(p_{B, 0|1}, p_{B, 1|0}, p_{V, 0|1}, p_{V, 1|0})\in A_{1-\alpha_{1}}.$ But this could be trivial. We need to think about when we want to minimize and when we want to maximize.  }

\textcolor{purple}{BZ 10/04: A guiding principle: We will be conducting a most optimistic analysis among ``safe and conservative" analyses making use of two negative control samples.}


\textcolor{blue}{Give two negative controls, we have two degrees of freedom only. We use $(p_{B, 0|1}, p_{V, 1|0})$ as two free nuisance parameters. For each given value of $(p_{B, 0|1}, p_{V, 1|0})$, we can use $A_{1-\alpha_{1}}$ to construct a valid confidence set for $(p_{B, 1|0}, p_{V, 0|1})$, denoted as $\mathcal{A}_{1-\alpha_{1}}(p_{B, 1|0}, p_{V, 0|1})$. Through looking at whether $\mathcal{A}_{1-\alpha_{1}}(p_{B, 1|0}, p_{V, 0|1})$ is empty or not, we can construct a joint lower bound for $(p_{B, 0|1}, p_{V, 1|0})$.  }

\textcolor{blue}{Try one-sided or two-sided for Theorem~\ref{thm: negative control}}.
\end{itemize}

\textcolor{violet}{Zhe: 
Given the false negative rates $(p_{B, 0|1}, p_{V, 0|1})$, a $100(1-\alpha_{1})\%$ confidence set for $(p_{B, 1|0}, p_{V, 1|0})$ based on the negative control is
\begin{equation*}
    A_{1-\alpha_{1}}=\{ p_{B, 1|0}\in[0, \min \{\widehat{p}^{N, *}_{B, 1},\widehat{p}^{(i), *}_{B, 1}\}], p_{V, 1|0}\in [0, \min \{\widehat{p}^{N, *}_{V, 1},\widehat{p}^{(i), *}_{V, 1}\}]: \overline{T}^{N}\in (-\infty, z_{1-\alpha_{1}}] \}.
\end{equation*}
% When $(p_{B, 0|1}, p_{V, 0|1})= (0,0)$, $T^{N}$ is monotonically decreasing with $p_{V, 1|0}$ and monotonically increasing with $p_{B, 1|0}$. 
% after adjustment, p-val goes higher
(Here we assume that the above form of confidence set is obtained by inverting the one-sided test $H_0: p_{B, 1|0} = b, p_{V, 1|0} = v$ against $H_0: p_{B, 1|0} < b, p_{V, 1|0} > v$?
Need to check monotonicity of $\overline{T}^{N}$ with respect to the nuisance parameters.)
To test $H_{0}^{i}$, we minimize the $p$-value in Theorem \ref{thm: study sample} over all plausible combinations of the nuisance parameters $( p_{B, 1|0}, p_{V, 1|0}) \in A_{1-\alpha_{1}}$. The rationale is that we want to identify the most significant evidence against the null hypothesis $H_{0}^{i}$, while ensuring that our findings are consistent with the observed negative controls data.
}


% Ex2: 43 --> 1

%To give a more explicit form for our strategy, henceforth, we assume the central limit theorem holds. We also assume that (1) the misclassification cases are independent across different cells; (2) outcomes (either true or measured) among different cells are independent before and after vaccination; (3) all the misclassification rates are equal among the study cells and negative control cells at each timepoint. (4) Under ground truth, we have $n_{0}^{\prime}=n_{1}^{\prime}=0$. 



\section{ICS data in COVPN 3008 Ubuntu Study}

Table \ref{tab: case study example} summarizes example data from one collected sample. Here, a CD4+ T cell is positive if it expresses IFN$\gamma$ and/or IL-2 against the antigen COV2 CON S1 before (baseline) and after receiving the primary mRNA COVID-19 vaccines. This is an example, judging from the two measurements of the negative control sample, that it appears that the change to misclassify a negative T cell as positive is higher for the post-vaccination measurement compared to the baseline measurement ($43/212,650$ vs $8/93883$).

\begin{table}[ht]
    \centering
    \begin{tabular}{cccccc} \hline
    &\multicolumn{2}{c}{Baseline} &\multicolumn{2}{c}{Post-vaccination}\\
         & Positive & Negative & Positive & Negative\\
        Participant $i$'s sample &  $31$ & $69,540 - 31$ &  $85$ & $93,562 - 85$ \\
       Negative control & $8$ & $93,883 - 8$ & $43$ & $212,650 - 43$ \\ \hline
    \end{tabular}
    \caption{Caption}
    \label{tab: case study example}
\end{table}

\begin{table}[ht]
    \centering
    \begin{tabular}{cccccc} \hline
    &\multicolumn{2}{c}{Baseline} &\multicolumn{2}{c}{Post-vaccination}\\
         & Positive & Negative & Positive & Negative\\
        Participant $i$'s sample &  $31$ & $69,540 - 31$ &  $70$ & $93,562 - 85$ \\
       Negative control & $8$ & $93,883 - 8$ & $60$ & $212,650 - 60$ \\ \hline
    \end{tabular}
    \caption{Caption}
    \label{tab: case study example}
\end{table}

\begin{table}[ht]
    \centering
    \begin{tabular}{cccccc} \hline
    &\multicolumn{2}{c}{Baseline} &\multicolumn{2}{c}{Post-vaccination}\\
         & Positive & Negative & Positive & Negative\\
        Participant $i$'s sample &  $31$ & $69,540 - 31$ &  $60$ & $93,562 - 85$ \\
       Negative control & $8$ & $93,883 - 8$ & $8$ & $212,650 - 60$ \\ \hline
    \end{tabular}
    \caption{Caption}
    \label{tab: case study example}
\end{table}

\textcolor{violet}{Zhe: 
Assuming both false negative rates  $(p_{B, 0|1}, p_{V, 0|1}) = (0,0)$, Figure \ref{fig:pvals} displays the $p$-values for testing hypothesis $H_{0}^{i}$ within a $95\%$ confidence set for $(p_{B, 1|0}, p_{V, 1|0})$ constructed using samples from the negative control. The results show that the negative control rejects both zero misclassification rates and the scenario of high false positives at baseline with low false positives post-vaccination. This is consistent with the increase in measured positivity of the negative controls at post-vaccination compared to baseline. All plausible values of 
 $(p_{B, 1|0}, p_{V, 1|0})$ yield significant $p$-values. Therefore, we are $95\%$ confident that participant $i$ is a responder, and this conclusion remains robust across various plausible false positive rates informed by the negative control.
}
\begin{figure}
    \centering
    \includegraphics[width=0.5\linewidth]{pvals.pdf}
    \caption{$p$-values over the confidence set of the nuisance parameters}
    \label{fig:pvals}
\end{figure}

\section{Incorporating paired control samples in determining a vaccine responder}\label{sec: method}
\subsection{One-sided misclassification}
\label{subsec: method one-sided misclassification}
Before introducing the generic procedure, to fix the idea, \textcolor{red}{we first consider a stylistic, one-sided misclassification scenario, where $p_{T_0, 0 \mid 1} = p_{T_1, 0 \mid 1} = 0$.} In other words, this is saying that a positive cell is not to be misclassified as negative at either $T_0$ or $T_1$. In this case, we have $p^{N}_{T_0, 1}= (p^{N, \ast}_{T_0, 1} - p_{T_0, 1\mid 0})/(1-p_{T_0, 1\mid 0})$ and $p^{N}_{T_1, 1}= (p^{N, \ast}_{T_1, 1} - p_{T_1, 1\mid 0})/(1-p_{T_1, 1\mid 0})$. Analogously, we have $p_{T_0, 1}= (p^{ \ast}_{T_0, 1} - p_{T_0, 1\mid 0})/(1-p_{T_0, 1\mid 0})$ and $p_{T_1, 1}= (p^{\ast}_{T_1, 1} - p_{T_1, 1\mid 0})/(1-p_{T_1, 1\mid 0})$.

We first consider the negative control samples at $T_0$ and $T_1$. Under fixed false positive rates $(p_{T_0, 1\mid 0}, p_{T_1, 1\mid 0})$, consider the test statistic 
  \begin{equation}\label{eq: T^N special case}
      T^{N}=\widehat{p}^{N}_{T_1, 1}-\widehat{p}^{N}_{T_0, 1} = \frac{\widehat{p}^{N, \ast}_{T_1, 1}-p_{T_1, 1\mid 0}}{1-p_{T_1, 1 \mid 0}} - \frac{\widehat{p}^{N, \ast}_{T_0, 1}-p_{T_0, 1\mid 0}}{1-p_{T_0, 1 \mid 0}},
  \end{equation}
  where $\widehat{p}^{N, \ast}_{T_1, 1} = n'_1/N'_1$ and $\widehat{p}^{N, \ast}_{T_0, 1} = n'_0/N'_0$ denote the sample proportion of positive cells in the negative control samples at $T_1$ and $T_0$, respectively. 

Consider testing the null hypothesis $H^N_0: p_{T_0, 1\mid 0} = b, p_{T_1, 1\mid 0} = v$ against the alternative \textcolor{red}{$H^N_1: p_{T_0, 1\mid 0} \neq b, p_{T_1, 1\mid 0} \neq v$ based on the test statistic $T^N$ in Equation \eqref{eq: T^N special case}.} Because we know $p^{N}_{T_0, 1} = p^{N}_{T_1, 1}$ \emph{a priori}, observed count data in the paired negative control samples can be used to make a confidence statement for the false positive rates at $T_0$ and $T_1$.

\begin{proposition}\label{prop: TN special case}
Suppose $p_{T_0, 0 \mid 1} = p_{T_1, 0 \mid 1} = 0$. Under fixed false positive rates at $T_0$ and $T_1$, we have
\begin{equation*}
      \overline{T}^{N}=  \frac{T^N }{\sqrt{\widehat{p}^{N}_{1}(1-\widehat{p}^{N}_{1}) \Big(\frac{1}{N_{1}^{\prime}}+\frac{1}{N_{0}^{\prime}}\Big) } }\xrightarrow{d} N(0,1),
\end{equation*}
where $T^N$ is given in \eqref{eq: T^N special case}, and
\begin{equation*}
\widehat{p}^{N}_{1}=\frac{N_{1}^{\prime}}{N_{0}^{\prime}+N_{1}^{\prime}}\times \frac{\widehat{p}^{N, \ast}_{T_1, 1}-p_{T_1, 1\mid 0}}{1-p_{T_1, 1 \mid 0}} + \frac{N_{0}^{\prime}}{N_{0}^{\prime}+N_{1}^{\prime}}\times \frac{\widehat{p}^{N, \ast}_{T_0, 1}-p_{T_0, 1\mid 0}}{1-p_{T_0, 1 \mid 0}}.
\end{equation*}
The null hypothesis $H^N_0: p_{T_0, 1\mid 0} = b, p_{T_1, 1\mid 0} = v$ against the alternative $H^N_1: p_{T_0, 1\mid 0} \neq b, p_{T_1, 1\mid 0} \neq v$ is rejected at level-$\alpha$ if XXX. By inverting the test, a one-sided confidence set of $(p_{T_0, 1\mid 0}, p_{T_1, 1\mid 0})$, denoted as $\mathcal{A}$, can be constructed as XXX.
\end{proposition}

Next, we turn our attention to two primary samples at $T_0$ and $T_1$. A study participant is considered a \emph{vaccine responder} at level-$\alpha$ if the null hypothesis
\begin{equation}
    \label{eq: primary null}
    H_0: p_{T_1, 1} = p_{T_0, 1}
\end{equation}
is rejected at level-$\alpha$ against the one-sided alternative $H_1: p_{T_1, 1} > p_{T_0, 1}$. Under fixed $(p_{T_0, 1\mid 0}, p_{T_1, 1\mid 0})$, we test the null hypothesis $H_0$ using the following test statistic $T$:
  \begin{equation}\label{eq: T special case}
      T = \widehat{p}_{T_1, 1}-\widehat{p}_{T_0, 1} = \frac{\widehat{p}^{\ast}_{T_1, 1} - p_{T_1, 1\mid 0}}{1-p_{T_1, 1\mid 0}} -\frac{\widehat{p}^{\ast}_{T_0, 1} - p_{T_0, 1\mid 0}}{1-p_{T_0, 1\mid 0}},
  \end{equation}
  where $\widehat{p}^{\ast}_{T_1, 1} = n_1/N_1$ and $\widehat{p}^{\ast}_{T_0, 1} = n_0/N_0$ denote the sample proportion of positive cells in participant $i$'s primary sample at $T_1$ and $T_0$, respectively.

\begin{proposition}
\label{prop: study sample special case}
    Under $H_{0}$ and given fixed false positive rates $(p_{T_0, 1\mid 0}, p_{T_1, 1\mid 0})$, we have 
    \begin{equation*}
      \overline{T}=  \frac{T}{\sqrt{\widehat{p}_{1}(1-\widehat{p}_{1}) \Big(\frac{1}{N_{1}}+\frac{1}{N_{0}}\Big) } }\xrightarrow{d} N(0,1),
    \end{equation*}
    where $T$ is given in \eqref{eq: T special case}, and
    \begin{equation*}
        \widehat{p}_{1}=\frac{N_{1}}{N_{0}+N_{1}}\times \frac{\widehat{p}^{\ast}_{T_1, 1}-p_{T_1, 1\mid 0}}{1-p_{T_1, 1\mid 0} }+\frac{N_{0}}{N_{0}+N_{1}}\times \frac{\widehat{p}^{\ast}_{T_0, 1}-p_{T_0, 1\mid 0}}{1-p_{T_0, 1\mid 0}}.
    \end{equation*}
A one-sided $p$-value for testing $H_{0}$ against $H_1$ given true false positive rates $(p_{T_0, 1\mid 0}, p_{T_1, 1\mid 0})$ is $1-\Phi(\overline{T})$, where $\Phi(\cdot)$ is the normal CDF.
\end{proposition}

Proposition \ref{prop: study sample special case} reduces to a usual two-sample analysis ignoring the paired negative controls and misclassification rates, that is, when $p_{T_1, 1\mid 0} = p_{T_0, 1\mid 0} = 0$.
